Attend2Pack: Bin Packing through Deep Reinforcement Learning with Attention

This paper seeks to tackle the bin packing problem (BPP) through a learning perspective. Building on self-attention-based encoding and deep reinforcement learning algorithms, we propose a new end-to-end learning model for this task of interest. By decomposing the combinatorial action space, as well as utilizing a new training technique denoted as prioritized oversampling, which is a general scheme to speed up on-policy learning, we achieve state-of-the-art performance in a range of experimental settings. Moreover, although the proposed approach attend2pack targets offline-BPP, we strip our method down to the strict online-BPP setting where it is also able to achieve state-of-the-art performance. With a set of ablation studies as well as comparisons against a range of previous works, we hope to offer as a valid baseline approach to this field of study.

==> secs/related.tex <==
\section{Related Work}
\label{sec:related}

%%%% previous pure heuristic approaches NOTE: might not be necessary

BPP is a famous problem in combinatorial optimization, it can be grouped into three groups,
1D-BPP, 2D-BPP, 3D-BPP, according to the items to be handled.
1D-BPP, a well-known NP-hard problem\cite{gareyComputersIntractabilityGuide1978}:
given a set of items with values (such as volume or weight),
pack them into a container with a maximum capacity to maximize the utilization of the capacity.
As a typical algorithm design paradigm, branch and bound (B\&B) is widely applied to enumerate the candidate solutions
\cite{martelloKnapsackProblemsAlgorithms1990}, \cite{schollBisonFastHybrid1997}, \cite{lysgaardNewBranchandcutAlgorithm2004}.
Integer Linear Programming(ILP), a widely used method in combinatorial optimization, has also applied to solve the BPP
\cite{dyckhoffNewLinearProgramming1981}, \cite{cambazardPropagatingBinPacking2010}, \cite{hadjsalemNewSymmetrylessILP2020}.
Additionally, Meta-Heuristic algorithms are also widely used, like \cite{abdel-bassetImprovedNatureInspired2018}, \cite{levineAntColonyOptimisation}, and \cite{lohSolvingOnedimensionalBin2008}.

% The BPP is proved that the best algorithm has the approximation ratio 3/2 and the time order $O(n)$, unless \emph{P=NP} \cite{zehmakanBinPackingProblem2015}. \cite{coffmanBinPackingApproximation1999} provides a comprehensive
% review of the approximation algorithms of BPP.

2D-BPP and 3D-BPP are more generalized versions of BPP. 2D-BPP/3D-BPP, which consider the dimensions of items,
is far more difficult than 1D-BPP because of the exponential action spaces.
Given $N$ items with different length, width and height $(l, w, h)$ and a container/bin with dimension $(L, W, H)$,
considering items orientations $O$, the full action space will be $N*O*L*W*H$,
Heuristics algorithms are widely used to solve 3D-BPP because of its efficiency, 
\cite{crainicExtremePointBasedHeuristics2008} presents a Extreme Point-based constructive heuristics method to reduce the action spaces efficiently,
items can only be placed in specific corner points of existing items in the container.
\cite{fanslauTreeSearchAlgorithm2010} introduces a general block-building approach, one or more items are first combined to build blocks, then
packed into the container, this approach achieved a significant improvements on performance.

Deep Reinforcement Learning(DRL) has achieved huge success on complex tasks, 
DeepMind showed impressive results on playing Atari game by using DRL\cite{mnihPlayingAtariDeep}.
Alpha Go\cite{silverMasteringGameGo2016} reached a milestone in 2015 that outperform a human professional Go player by introducing a Neural MCTS method.
\cite{bello2016neural} tackled the classic combinatorial optimization problems traveling salesman problem (TSP) 
by using neural networks and reinforcement learning.
\cite{kool2018attention} shows significant performance improvement by proposing a model based on Pointer Network \cite{vinyals2015pointer}.
These achievements show that DRL has huge potential advantages on combinatorial optimization,
Ranked Reward\cite{laterre2018ranked} applied the Neural MCTS approach on 2D-BPP and 3D-BPP,
the results showed that the performance is better than pure MCTS and GUROBI solver especially when handles large number of items.
\cite{duan2019multi} applied DRL to deal with the sequential decision problem in offline 3D-BPP.
\cite{zhao2020online} introduces a prediction-and-projection method to solve online 3D-BPP (palletizing). 
\cite{tanakaSimultaneousPlanningItem} leverages DRL to solve the simultaneous item picking and placing problem.

%%%% previous learning approaches

%% online bin packing

% \cite{zhao2020online}
% are their seqs sorted???
% fixed/random sequence,
% learn the placement strategy
% pg.3 as the complexity of bpp decreases drastically for bigger items,
% we further constrain the sizes of all items to be
% $l_i<=L/2$


% \cite{young2020smart}
% also does online bin packing,
% but puts the focus on building the autonomous bin packing system,
% measuring the dimensions of incoming objects in real-time and placing objects into containers according to a predefined heuristic.


%% learning the sequence, place with heuristic


%% 
% \hl{ranked reward}???
% what are their results???

% \cite{duan2019multi}


%%%% multi-agent 

